Infinitely Divisible Noise for Differential Privacy: Nearly Optimal Error in the High $\varepsilon$ Regime

Differential privacy (DP) can be achieved in a distributed manner, where multiple parties add independent noise such that their sum protects the overall dataset with DP. A common technique here is for each party to sample their noise from the decomposition of an infinitely divisible distribution. We analyze two mechanisms in this setting: 1) the generalized discrete Laplace (GDL) mechanism, whose distribution (which is closed under summation) follows from differences of i.i.d. negative binomial shares, and 2) the multi-scale discrete Laplace (MSDLap) mechanism, a novel mechanism following the sum of multiple i.i.d. discrete Laplace shares at different scales. For $\varepsilon \geq 1$, our mechanisms can be parameterized to have $O\left(\Delta^3 e^{-\varepsilon}\right)$ and $O\left(\min\left(\Delta^3 e^{-\varepsilon}, \Delta^2 e^{-2\varepsilon/3}\right)\right)$ MSE, respectively, where $\Delta$ denote the sensitivity; the latter bound matches known optimality results. We also show a transformation from the discrete setting to the continuous setting, which allows us to transform both mechanisms to the continuous setting and thereby achieve the optimal $O\left(\Delta^2 e^{-2\varepsilon / 3}\right)$ MSE. To our knowledge, these are the first infinitely divisible additive noise mechanisms that achieve order-optimal MSE under pure DP, so our work shows formally there is no separation in utility when query-independent noise adding mechanisms are restricted to infinitely divisible noise. For the continuous setting, our result improves upon the Arete mechanism from [Pagh and Stausholm, ALT 2022] which gives an MSE of $O\left(\Delta^2 e^{-\varepsilon/4}\right)$. Furthermore, we give an exact sampler tuned to efficiently implement the MSDLap mechanism, and we apply our results to improve a state of the art multi-message shuffle DP protocol in the high $\varepsilon$ regime.

==> old-work/arete/old-arete-work.tex <==
\section{Arete mechanism}

The Arete mechanism was introduced and studied in \cite{pagh2022infinitely}. There, the authors showed that the
mechanism with additive Arete noise is $\eps$-differentially private and enjoys $O(\Delta^2 e^{-\eps/4})$ variance.
In this section, we show that it actually achives the optimal $O(\Delta^2 e^{-2\eps/3})$ variance with an improved
parameterization and analysis.

\begin{definition}[\cite{pagh2022infinitely}]
    For parameters $\alpha > 0$, $\beta > 0$, and $\lambda > 0$ let $Z \sim \Gamma(\alpha, \beta) - \Gamma(\alpha, \beta) + \Lap(\lambda)$.
    Then $Z \sim \Arete(\alpha, \beta, \lambda)$.
\end{definition}

Unfortunately, the Arete distribution's PDF has no known closed form expression. This makes it quite difficult to tightly characterize its privacy. To help, we will introduce two auxiliary distributions, $\Arete_u$ and $\Gamma-\Gamma$, and also show a analytical form for the Arete's PDF at 0. For PDF evaluation we
make use of symbolic integration from Mathematica.

\begin{equation}
    f_{\Arete(\alpha,\beta, \lambda)}(0) =
    \frac{1}{2} \sec(\pi \beta) \left(
        \lambda^{2\beta -1} \left(\alpha^2 - \lambda^2\right)^{-\beta} -
        \frac{\sqrt{\pi} \HG{\frac{1}{2}}{1}{\frac{3}{2}-\beta}{\frac{\lambda^2}{\alpha^2}}}
            {\alpha \Gamma(\beta) \Gamma(\frac{3}{2}-\beta)}
    \right)
\end{equation}
    
\begin{definition}
    For parameters $\alpha > 0$, $\beta > 0$, and $\lambda > 0$ let $Z \sim \Gamma(\alpha, \beta) + \Lap(\lambda)$.
    Then $Z \sim \Arete_u(\alpha, \beta, \lambda)$. It's PDF is
    \begin{align*}
    &f_{\Arete_u(\alpha, \beta, \lambda)}(x) =\\ 
        &\begin{cases}
            \frac{1}{2}e^{x/\lambda} \lambda^{\alpha - 1} (\beta + \lambda)^{-\alpha} & x \le 0\\
            \frac{e^{-x/\lambda} \beta^{-\alpha}(1-\frac{\beta}{\lambda})^{-\alpha}}
                 {2\lambda \Gamma(\alpha)} 
            \left(
                e^{2 x / \lambda} x^\alpha (1-\beta/\lambda)^\alpha \Ei_{1-\alpha}(x(\frac{1}{\beta}+\frac{1}{\lambda})) +
                \beta^\alpha \left(\Gamma(\alpha) - 
                \Gamma(\alpha, x(\frac{1}{\beta}-\frac{1}{\lambda}))\right)
            \right)
            & x > 0
        \end{cases}
    \end{align*}

Where $\Ei_n(z)=\int_1^\infty e^{-z t} / t^n dt$ is the exponential integral function, and $\Gamma(a,b)$ is the incomplete gamma function.
\end{definition}
The $\Arete_u$ distribution can be considered a "one-sided" version of the Arete distribution, as it does not include the negative $\Gamma$ term.

\begin{lemma}\label{lem:areteu-logconvex}
$f_{Arete_u(\alpha, \beta, \lambda)}(x)$ is log-convex on $(t, \infty)$ where
$t \ge \max\left(0, 
              \frac{(\alpha - 1)\beta \lambda}{\beta + \lambda},
              -\frac{(\alpha - 1)\beta \lambda}{\beta - \lambda} 
            \right)$.
\end{lemma}
\begin{proof}
The sum of log-convex functions is log-convex, so consider breaking $f_{\Arete_u(\alpha, \beta, \lambda)}(x) = f(x) + h(x)$ where:
\begin{align*}
f(x) &= 
    \frac{\beta^{-\alpha}}
                 {2\lambda \Gamma(\alpha)}
    e^{x /\lambda} x^\alpha
    \Ei_{1-\alpha}\left(x\left(\frac{1}{\beta}+\frac{1}{\lambda}\right)\right)
    \\
    &= \frac{\beta^{-\alpha}}
                 {2\lambda \Gamma(\alpha)}
        e^{x/\lambda}
        \left(\frac{1}{\beta}+\frac{1}{\lambda}\right)^{-\alpha}
        \Gamma\left(\alpha, 
               x\left(\frac{1}{\beta}+\frac{1}{\lambda}\right))\right)\\\\
h(x) &= 
    \frac{e^{-x/\lambda} (1-\frac{\beta}{\lambda})^{-\alpha}}
                 {2\lambda \Gamma(\alpha)}
    \left(
    \Gamma(\alpha) - \Gamma(\alpha, x(\frac{1}{\beta}-\frac{1}{\lambda}))
    \right)\\\\
\end{align*}

The incomplete gamma function $\Gamma(a, x)$ is log-convex when $x - a + 1 \ge 0$ \cite{}.
Therefore $f(x)$ is log-convex when:

\begin{align*}
x\left(\frac{1}{\beta}+\frac{1}{\lambda}\right) - \alpha + 1 &\ge 0\\
x &\ge \frac{\alpha - 1}{\frac{1}{\beta}-\frac{1}{\lambda}} \\
 &= \frac{(\alpha - 1)\beta \lambda}{\beta + \lambda} 
\end{align*}

\todo{Show $h(x)$ is log-convex. It is tricky}

\end{proof}

\begin{lemma}\label{lem:areteu-larger}
For $x > \max\left(
              \frac{(\alpha - 1)\beta \lambda}{\beta + \lambda},
              -\frac{(\alpha - 1)\beta \lambda}{\beta - \lambda} 
            \right)$:

$$
    \frac{f_{\Arete(\alpha,\beta,\lambda)}(x)}{f_{\Arete(\alpha,\beta,\lambda)}(x+1)}
    \le 
    \frac{f_{\Arete_u(\alpha,\beta,\lambda)}(x)}{f_{\Arete_u(\alpha,\beta,\lambda)}(x+1)}
$$
\end{lemma}
\begin{proof}
We will use the convolution identity:
\begin{align*}
    f_{\Arete(\alpha, \beta, \lambda)}(x) &= \int_{-\infty}^0 f_{-\Gamma(\alpha, \beta)}(\tau) f_{\Arete_u(\alpha,\beta,\lambda)}(x-\tau) d\tau \\
    &= \int_{0}^\infty f_{\Gamma(\alpha, \beta)}(\tau) f_{\Arete_u(\alpha,\beta,\lambda)}(x+\tau) d\tau \\
\end{align*}

\begin{align*}
\frac{f_{\Arete(\alpha,\beta,\lambda)}(x)}{f_{\Arete_u(\alpha,\beta,\lambda)}(x)}
&= \frac{\int_{0}^\infty f_{\Gamma(\alpha, \beta)}(\tau) f_{\Arete_u(\alpha,\beta,\lambda)}(x+\tau) d\tau }{f_{\Arete_u(\alpha,\beta,\lambda)}(x)}\\
&= \int_{0}^\infty 
    f_{\Gamma(\alpha, \beta)}(\tau) 
    \frac{f_{\Arete_u(\alpha,\beta,\lambda)}(x+\tau)}
    {f_{\Arete_u(\alpha,\beta,\lambda)}(x)} d\tau\\
&\le \int_{0}^\infty 
    f_{\Gamma(\alpha, \beta)}(\tau) 
    \frac{f_{\Arete_u(\alpha,\beta,\lambda)}(x+\tau+1)}
    {f_{\Arete_u(\alpha,\beta,\lambda)}(x+1)} d\tau & \text{\Cref{lem:logconvex} and \Cref{lem:areteu-logconvex}}\\
&= \frac{f_{\Arete(\alpha,\beta,\lambda)}(x+1)}{f_{\Arete_u(\alpha,\beta,\lambda)}(x+1)}
\end{align*}

The result follows from re-arranging the inequality.

\todo{I think we can use this general proof technique to show that any $D-D$ distribution for $D$ log-convex (and with finite PDF everywhere) is differentially private and the dominating pair is $f_D(0)/f_D(1)$. From
some other results we know all log-convex positive distributions are infinitely divisible...}

\end{proof}

\begin{definition}[\cite{pagh2022infinitely}]
    For parameters $0 < \alpha < \frac{1}{2}$, $\beta > 0$, let $Z \sim \Gamma(\alpha, \beta) - \Gamma(\alpha, \beta)$.
    Then $Z \sim \Gamma-\Gamma(\alpha, \beta)$. It's PDF is
\begin{align*}
f_{\Gamma-\Gamma(\alpha, \beta)} =
\begin{cases}
    \frac{1}{\sqrt{\pi} \Gamma(\alpha)} 2^{-\alpha + \frac{1}{2}} x^{\alpha - \frac{1}{2}} \left(\frac{1}{\beta^2}\right)^\alpha
    \left(\frac{1}{\beta}\right)^{-\alpha + \frac{1}{2}} \K_{\alpha - \frac{1}{2}}(\frac{x}{\beta})
    & x > 0\\
    \frac{1}{\sqrt{\pi} \Gamma(\alpha)} 2^{-\alpha + \frac{1}{2}} (-x)^{\alpha - \frac{1}{2}} \left(\frac{1}{\beta^2}\right)^\alpha
    \left(\frac{1}{\beta}\right)^{-\alpha + \frac{1}{2}} \K_{\alpha - \frac{1}{2}}(-\frac{x}{\beta})
    & x < 0\\
    \infty & x = 0
\end{cases}
\end{align*}

Where $\K_n(z)$ is the modified Bessel function of the second kind.
\end{definition}


\begin{lemma}\label{lem:gg-lower}
For $m > ?$\todo{},
$f_{\Gamma-\Gamma(\alpha, \beta)}(m) \le f_{\Arete(\alpha, \beta, \lambda)}(m)$
\end{lemma}
\begin{proof}
Since the $\Gamma-\Gamma$ distribution is fast decreasing, the intuition is that
convolving with a Laplace PDF will increase the PDF at $m$, since there is much more  $\Gamma-\Gamma$ mass nearer to 0.

\begin{align*}
f_{\Arete(\alpha, \beta, \lambda)}(m) &=
    \int_{-\infty}^\infty f_{\Lap(\lambda)}(\tau)f_{\Gamma-\Gamma(\alpha,\beta)}(m -\tau)d\tau\\
&= 
    \int_{-\infty}^0 f_{\Lap(\lambda)}(\tau)f_{\Gamma-\Gamma(\alpha,\beta)}(m -\tau)d\tau +
    \int_{0}^\infty f_{\Lap(\lambda)}(\tau)f_{\Gamma-\Gamma(\alpha,\beta)}(m-\tau)d\tau\\
&= 
    \int_{0}^\infty f_{\Lap(\lambda)}(\tau)f_{\Gamma-\Gamma(\alpha,\beta)}(m+\tau)d\tau +
    \int_{0}^\infty f_{\Lap(\lambda)}(\tau)f_{\Gamma-\Gamma(\alpha,\beta)}(m -\tau)d\tau\\
\end{align*}
\todo{Finish the proof}
\end{proof}


\begin{lemma}\label{lem:arete-ratio-bound}
    For $x \ge 0$,
    $$
    \frac{f_{\Arete(\alpha, \beta,\lambda)}(x)}{f_{\Arete(\alpha, \beta,\lambda)}(x+1)}
    \le 
    \max \left(
    \frac{f_{\Arete_u(\alpha, \beta,\lambda)}(t)}{f_{\Arete_u(\alpha, \beta,\lambda)}(t +1)},
    \frac{f_{\Arete(\alpha, \beta,\lambda)}(0)}{f_{\Gamma-\Gamma(\alpha, \beta)}(t+1)}
    \right)
    $$
Where
$t = \max\left(
              \frac{(\alpha - 1)\beta \lambda}{\beta + \lambda},
              -\frac{(\alpha - 1)\beta \lambda}{\beta - \lambda} 
            \right)$.
\todo{some restriction when Gamma-Gamma is a lower bound from \Cref{lem:gg-lower}}
\end{lemma}
\begin{proof}

Let $x_{max}$ be the value of $x$ that maximizes $\frac{f_{\Arete(\alpha, \beta,\lambda)}(x)}{f_{\Arete(\alpha, \beta,\lambda)}(x+1)}$. There are two cases to
consider:

\begin{enumerate}
\item $0 \le x_{max} \le t$. Here
\begin{align*}
    \frac{f_{\Arete(\alpha, \beta,\lambda)}(x_{max})}{f_{\Arete(\alpha, \beta,\lambda)}(x_{max}+1)}
    &\le
    \frac{f_{\Arete(\alpha, \beta,\lambda)}(0)}{f_{\Arete(\alpha, \beta,\lambda)}(t+1)}& \text{ by $\Arete$ decreasing}\\
&\le \frac{f_{\Arete(\alpha, \beta,\lambda)}(0)}{f_{\Gamma-\Gamma(\alpha, \beta)}(t+1)} & \text{\Cref{lem:gg-lower}}\\
\end{align*}

\item $x_{max} > t$. In this case 
\begin{align*}
    \frac{f_{\Arete(\alpha, \beta,\lambda)}(x)}{f_{\Arete(\alpha, \beta,\lambda)}(x+1)}
    &\le 
    \frac{f_{\Arete_u(\alpha, \beta,\lambda)}(t)}{f_{\Arete_u(\alpha, \beta,\lambda)}(t +1)} & \text{\Cref{lem:areteu-larger}}\\
\end{align*}

\end{enumerate}
\end{proof}

\begin{theorem}
    Let $\Delta \ge 1$, $\eps > 3 \log(2) / 2$ \todo{we need the $\Gamma-\Gamma$ restrictions on epsilon} and $q: X^d \to \mathbb{R}$ such that $|q(x)-q(x')|\le \Delta$ for all $x, x' \in X^d$
    which differ on a single entry. Define the randomized algorithm $M: X^d \to \mathbb{R}$ by $M(x) = \Delta (q(x)/\Delta + Z)$
    where $Z \sim \Arete(\alpha, \beta, \lambda)$.
    Then $M$ with $\alpha = e^{-2 \eps / 3}$, $\beta = (1+t) \frac{1}{\log 2}$, and $\lambda = (1+t) e^{-\eps / 3}$ where $t \ge \frac{e^{2 \eps / 3} - 1}{1+e^\eps - e^{2\eps / 3} (1 + \log(2))}$
    satisfies $\eps$-differential privacy and the noise has $O(\Delta^2 e^{-2\eps/3})$ variance.
\end{theorem}
\begin{proof}

For $\Delta > 1$, we use DP postprocessing to show that the scaled
mechanism with sensitivity $1$ is private, so the rescaled mechanism is also private. Thus it suffices to consider $\Delta = 1$.


The restriction on $\eps$ comes from our need for $\alpha < \frac{1}{2}$.
Set
\begin{align*}
t &\ge \max\left(
              \frac{(\alpha - 1)\beta \lambda}{\beta + \lambda},
              -\frac{(\alpha - 1)\beta \lambda}{\beta - \lambda} 
            \right)\\
&= \max\left(
              \frac{(e^{-2\eps/3} - 1) (1+t)}{e^\eps - e^{2 \eps / 3} \log(2)},
              -\frac{(e^{-2\eps/3} - 1) (1+t)}{e^\eps + e^{2 \eps / 3} \log(2)}
            \right)\\
&= \frac{(e^{-2\eps/3} - 1) (1+t)}{e^\eps - e^{2 \eps / 3} \log(2)}
\end{align*}

Solving for $t$ yields
$$
t \ge \frac{e^{2 \eps / 3} - 1}{1+e^\eps - e^{2\eps / 3} (1 + \log(2))}
$$

From \Cref{lem:arete-ratio-bound} it suffices to show that

$$
\log \left(
    \max \left(
    \frac{f_{\Arete_u(\alpha, \beta,\lambda)}(t)}{f_{\Arete_u(\alpha, \beta,\lambda)}(t +1)},
    \frac{f_{\Arete(\alpha, \beta,\lambda)}(0)}{f_{\Gamma-\Gamma(\alpha, \beta)}(t+1)}
    \right)
\right)
\le \eps
$$

\todo{do show this. If not possible think about how we can do this w/ computer assist}

To show the variance:

\begin{align*}
Var[\Delta Arete(\alpha, \beta, \lambda)] &= 2(\alpha \beta^2 + \lambda^2) \Delta^2 \\
&= 2(e^{-2 \eps / 3} \frac{1}{\log^2 2} + e^{-2 \eps / 3}) t^2 \Delta^2\\
&= O(\Delta^2 e^{-2 \eps / 3})
\end{align*}

\end{proof}

\begin{figure}[htbp]
  \centering
  \includesvg[inkscapelatex=false, width = 425pt]{fig2.svg}
  \caption{The variance of the Arete distribution vs. a Continuous Staircase baseline. Note well the restrictions on $\eps$ for each Arete analysis.}
\end{figure}




==> old-work/sampling-app.tex <==
\subsection{A less restrictive $\NB$ sampler}\label{sec:alternative-nb-sample}
\begin{algorithm}
    \caption{Negative binomial sampling \cite[Algorithm 4.1]{heaukulani2019black}}
    \label{alg:nb-sample-rational}
\begin{flushleft}
\textbf{Input}: $r = a/b \in \mathbb{Q}$, $\gamma \in \mathbb{Q}$
\textbf{Output}: A sample from $\NB(r, 1-e^{-\gamma})$
\begin{algorithmic}[1] %[1] enables line numbers
\Loop \Comment{Rejection sampler proposing $\NB(\lceil r \rceil, p)$}
\State Sample $w \gets \Call{SampleIntegerNB}{\lceil r \rceil, 1 - e^{-\gamma}}$ \Comment{Use SampleIntegerNB}
\State $A_w \gets (r)_w / (\lceil r \rceil)_w$ \Comment $(x)_n$ is the Pochhammer symbol
\State Sample $accept \gets \Ber(A_w)$
\If{accept}
    \State \textbf{return} w
\EndIf
\EndLoop
\Procedure{SampleIntegerNB}{$r$, $\gamma$}
\State $failures \gets 0$
\State $successes \gets 0$
\Loop
    \State Sample $A \gets \Ber(1 - e^{-\gamma})$
    \If{$A = 1$}
        \State $successes \gets successes + 1$
        \If{$successes = r$} break \EndIf
    \Else
        \State $failures \gets failures + 1$
    \EndIf
\EndLoop
\State \textbf{return} $failures$
\EndProcedure
\end{algorithmic}
\end{flushleft}
\end{algorithm}


\begin{proposition}\label{prop:nb-sample-rational}
For input $r \in \mathbb{Q}$, and $p = 1-e^{-\gamma}$ for $\gamma \in \mathbb{Q}$, the procedure described in \Cref{alg:nb-sample-rational} returns one sample from $NB(r, p)$ and completes in $O(r / p^2)$ steps in expectation.
\end{proposition}
\begin{proof}
We begin with analyzing the integer procedure. Fix an output $k \ge 0$. This means there are $k$ failures and $r$ successes, and $\binom{k + r - 1}{k}$ possible ways the
algorithm could generate the output (by counting the arrangements of $r-1$ successes and $k$ failures).
Therefore the probability of seeing $k$ is

\begin{align*}
\binom{k + r - 1}{k}p^{r}(1-p)^k = f_{\NB(r, p)}.
\end{align*}

It is clear that the procedure takes $O(successes + failures)$ steps, which is $O(r + \E[\NB(r, p)]) = O(r/p)$.
Next we analyze the outer loop which handles rational values of $r$ using a standard accept-reject approach:
\begin{itemize}
    \item The proposal distribution is $\NB(\lceil r \rceil, p)$.
    \item The target distribution is $\NB(r ,p)$.
    \item The constant $C = p^{r - \lceil r \rceil}$ 
\end{itemize}
The above ensures that a proposed sample $w$ is accepted with probability
\begin{align*}
    A_w &= \frac{f_{\NB(r ,p)}(w)}{C\cdot f_{\NB(\lceil r \rceil, p)}(w)}
    = \frac{\frac{\Gamma(w + r)}{\Gamma(r)\Gamma(w+1)} p^r}{C\cdot \frac{\Gamma(w + \lceil r \rceil)}{\Gamma(\lceil r \rceil)\Gamma(w+1)} p^{\lceil r \rceil}}\\
    &= \frac{\Gamma(w+r)\Gamma(\lceil r \rceil)}{\Gamma(w+\lceil r \rceil)\Gamma(r)}\\
    &= \frac{(r)_w}{(\lceil r \rceil)_w}.
\end{align*}
The last equality follows from the identity $(x)_n = \frac{\Gamma(x + n)}{\Gamma(x)}$. The number of trials is a geometric distribution with success probability
\begin{align*}
\mathop{\mathbb{E}}_{w \sim \NB(\lceil r \rceil, p)}\left[\frac{(r)_w}{(\lceil r \rceil)_w}\right]
&= \mathop{\mathbb{E}}_{w \sim \NB(r, p)}\left[\frac{1}{C}\right]
= \frac{1}{C}
\end{align*}
Therefore the expected number of trials is $C = O(1/p)$,
and the result follows.
\end{proof}


\begin{algorithm}[t]
    \caption{Negative binomial sampling}
    \label{alg:nb-sample-inverse}
\begin{flushleft}
\textbf{Input}: $r \in \mathbb{Q}$, $0 < p < 1 \in \mathbb{Q}$
\textbf{Output}: A sample from $\NB(r, p)$
\begin{algorithmic}[1] %[1] enables line numbers
\Loop \Comment{Rejection sampler proposing $\NB(\lceil r \rceil, p)$}
    \State Sample $w \gets \Call{SampleIntegerNB}{\lceil r \rceil, p}$
    \State $A_w \gets (r)_w / (\lceil r \rceil)_w$
    \State Sample $accept \gets \Ber(A_w)$
    \If{$accept$} \textbf{return} $w$ \EndIf
\EndLoop
\Procedure{SampleIntegerNB}{r, p}
\State $coeff \gets 1$
\State $prevsum = 0$
\For{$k$ in $\{0, 1, \cdots, \infty\}$}
    \State $f = coeff \cdot p^r \cdot (1-p)^k$
            \Comment{$coeff = \binom{k+r-1}{k}$}
    \State Sample $A \gets \Ber\left(\frac{f}{1-prevsum}\right)$
        \Comment{$prevsum = \sum_{i=0}^{k-1} f(i)$}
    \If{$A = 1$} \textbf{return $k$} \EndIf
    \State $prevsum \gets prevsum + f$
    \State $coeff \gets coeff \cdot \frac{r+k}{1+k}$
\EndFor
\EndProcedure
\end{algorithmic}
\end{flushleft}
\end{algorithm}

\begin{proposition}\label{prop:nb-sample-inverse}
For input $r \in \mathbb{Q}$, and $0 < p < 1 \in \mathbb{Q}$, the procedure described in \Cref{alg:nb-sample} returns one sample from $NB(r, p)$ and completes in $O(r (1-p)/p^2)$ steps in expectation.
\end{proposition}
\begin{proof}
    We begin by analyzing the case for integer $r$, which amounts to analyzing $\Call{SampleIntegerNB}{}$. Let $K$ be the random variable describing the output of $\Call{SampleIntegerNB}{}$ and let $f = f_{\NB(r,p)}$ for brevity.
    For correctness, we proceed with induction on $k$, where the base case of $\pr{K=0} = f(0)$ is trivial. For the induction step, note
    \begin{align*}
    \pr{K = k} &= \pr{K > k-1} \cdot \frac{f(k)}{1 - \sum_{i=0}^{k-1} f(i)}\\
    &= \left(1-\sum_{i=0}^{k-1} f(i)\right) \cdot \frac{f(k)}{1 - \sum_{i=0}^{k-1} f(i)}\\
    &= f(k)
    \end{align*}
    In expectation, the algorithm terminates in $\E[K] = \E[\NB(r, p)] = r (1-p)/p$ iterations and each iteration completes in $O(1)$ steps.

    Next we analyze the outer loop which handles rational values of $r$ using a standard accept-reject approach \cite{monte-carlo-book}:
    \begin{itemize}
        \item The proposal distribution is $\NB(\lceil r \rceil, p)$.
        \item The target distribution is $\NB(r ,p)$.
        \item The constant $C = p^{r - \lceil r \rceil}$ 
    \end{itemize}
        The above ensures that a proposed sample $w$ is accepted with probability
    \begin{align*}
        A_w &= \frac{f_{\NB(r ,p)}(w)}{C\cdot f_{\NB(\lceil r \rceil, p)}(w)}
        = \frac{\frac{\Gamma(w + r)}{\Gamma(r)\Gamma(w+1)} p^r}{C\cdot \frac{\Gamma(w + \lceil r \rceil)}{\Gamma(\lceil r \rceil)\Gamma(w+1)} p^{\lceil r \rceil}}\\
        &= \frac{\Gamma(w+r)\Gamma(\lceil r \rceil)}{\Gamma(w+\lceil r \rceil)\Gamma(r)}\\
        &= \frac{(r)_w}{(\lceil r \rceil)_w}.
    \end{align*}
    The last equality follows from the identity \Cref{eq:pochhammer}. The number of trials follows a geometric distribution with success probability
    \begin{align*}
    \mathop{\mathbb{E}}_{w \sim \NB(\lceil r \rceil, p)}\left[\frac{(r)_w}{(\lceil r \rceil)_w}\right]
    &= \mathop{\mathbb{E}}_{w \sim \NB(r, p)}\left[\frac{1}{C}\right]
    = \frac{1}{C}
    \end{align*}
    Therefore the expected number of trials is $C = O(1/p)$,
    and the result follows.
\end{proof}

\begin{remark}
\Cref{alg:nb-sample} can only handle rational values of $p$, which precludes
setting $p = 1-e^{\eps}$ for rational $\eps$, though rounding $1-e^{-\eps}$ to a larger rational should have minimal impact to accuracy in practice. This issue is easily resolved by using 
the standard waiting-time negative binomial sampler, which can leverage the $\Ber(e^{-\gamma})$ sampler from \cite{canonne2020discrete}. However, this sampler takes time linear in $r$.
\end{remark}

